First measurement using elliptically polarized photons of the double-polarization observable $E$ for $\gamma p \to p \pi^0$ and $\gamma p \to n \pi^+$

We report the measurement of the helicity asymmetry $E$ for the $p\pi^0$ and $n\pi^+$ final states using, for the first time, an elliptically polarized photon beam in combination with a longitudinally polarized target at the Crystal Ball experiment at MAMI. The results agree very well with data that were taken with a circularly polarized photon beam, showing that it is possible to simultaneously measure polarization observables that require linearly (e.g.~$G$) and circularly polarized photons (e.g.~$E$) and a longitudinally polarized target. The new data cover a photon energy range 270 - 1400 MeV for the $p\pi^0$ final state (230 - 842 MeV for the $n\pi^+$ final state) and the full range of pion polar angles, $\theta$, providing the most precise measurement of the observable $E$. A moment analysis gives a clear observation of the $p\eta$ cusp in the $p\pi^0$ final state.

==> acknowledgement.tex <==
% acknowledgement_APS_full_names.tex             18 June 2018
%
% Acknowledgement paragraph in English of Oct. 15, 2014 for APS journals
We thank Prof. Richard T. Jones for the fruitful discussions regarding the calculation of the circular polarization degree. We wish to further acknowledge the outstanding support of the accelerator group and  operators of MAMI. This work was supported by Schweizerischer Nationalfonds (200020-156983, 132799, 121781, 117601), Deutsche Forschungsgemeinschaft (SFB443,  SFB1044, SFB/TR16), the INFN-Italy, the European Community-Research Infrastructure Activity under FP7 programme (Hadron Physics, grant agreement No. 227431), the U.~K.~Science and Technology Facilities Council grants ST/J000175/1, ST/G008604/1, ST/G008582/1, ST/J00006X/1, ST/V001035/1 ST/V002570/1, ST/P004385/2, ST/T002077/1, and ST/L00478X/2, the Natural Sciences and Engineering Research Council (NSERC, FRN: SAPPJ-2015-00023), Canada. This material is based upon work also supported by the U.S. Department of Energy, Office of Science, Office of Nuclear Physics Research Division, under Award Numbers DE-FG02-99-ER41110, DE-FG02-88ER40415, DE-FG02-01-ER41194, DE-SC0014323 and DE-SC0016583 and by the National Science Foundation, under Grant Nos. PHY-1039130 andIIA-1358175.

%


==> author_list.tex <==
% remove these 3 lines before journal submittal.
%\centerline{author list dated 18 June 2018}
% end removal before journal submittal
%
%\affiliation{Helmholtz-Institut f\"ur Strahlen- und Kernphysik, Universit\"at Bonn, Germany}

%
%\author{F.N.~Afzal...} \affiliation{Helmholtz-Institut f\"ur Strahlen- und Kernphysik, Universit\"at Bonn, Germany}

%\affiliation{\HISKP}
\affiliation{\HISKP}%5
\affiliation{\GLASGOW}%7
\affiliation{\BASEL}%3
\affiliation{\MAINZ}%4
\affiliation{\REGINA}%2
\affiliation{\YORK}%1
\affiliation{\KENT}%6
\affiliation{\DUBNA}%8
\affiliation{\PAVIAINFN}%9
\affiliation{\WASHINGTON}%10
\affiliation{\HALIFAXCANADA}%11
\affiliation{\PAVIA}%12
\affiliation{\GIESSEN}%13
\affiliation{\BOCHUM}
\affiliation{\MOSCOW}%14
\affiliation{\MOUNTALLISON}%15
\affiliation{\ZAGREB}%16
\affiliation{\MASSACHUSETTS}%17
%\affiliation{\LA}%18
%\affiliation{\JERUSALEM}%19
%\affiliation{\NEWJERSEY}%20
%\affiliation{\JLAB}%21 

\author{F.~Afzal}\email[Corresponding author: ]{afzal@hiskp.uni-bonn.de}\affiliation{\HISKP}
\author{K.~Spieker}\affiliation{\HISKP}
\author{P.~Hurck}\affiliation{\GLASGOW}
\author{S. Abt}\affiliation{\BASEL}
\author{P. Achenbach}\affiliation{\MAINZ}
\author{P. Adlarson}\affiliation{\MAINZ}
\author{Z. Ahmed}\affiliation{\REGINA}
\author{C.S. Akondi}\affiliation{\KENT}
\author{J.R.M. Annand}\affiliation{\GLASGOW}
\author{H.J. Arends}\affiliation{\MAINZ}
\author{M. Bashkanov}\affiliation{\YORK}
\author{R. Beck}\affiliation{\HISKP}
\author{M. Biroth}\affiliation{\MAINZ}
\author{N. Borisov}\affiliation{\DUBNA}
\author{A. Braghieri}\affiliation{\PAVIAINFN}
\author{W.J. Briscoe}\affiliation{\WASHINGTON}
\author{F. Cividini}\affiliation{\MAINZ}
\author{C. Collicott}\affiliation{\HALIFAXCANADA}
\author{S. Costanza}\affiliation{\PAVIA}\affiliation{\PAVIAINFN}
\author{A. Denig}\affiliation{\MAINZ}
\author{M. Dieterle}\affiliation{\BASEL}
\author{E.J. Downie}\affiliation{\WASHINGTON}
\author{P. Drexler}\affiliation{\MAINZ}\affiliation{\GIESSEN}
\author{S. Fegan}\affiliation{\YORK}
\author{S. Gardner}\affiliation{\GLASGOW}
\author{D.I. Glazier}\affiliation{\GLASGOW}
\author{I. Gorodnov}\affiliation{\DUBNA}
\author{W. Gradl}\affiliation{\MAINZ}
\author{D. Gurevich}\affiliation{\MOSCOW}
\author{L. Heijkenskj\"old}\affiliation{\MAINZ}
\author{D. Hornidge}\affiliation{\MOUNTALLISON}
\author{G.M. Huber}\affiliation{\REGINA}
\author{V.L. Kashevarov}\affiliation{\MAINZ}\affiliation{\DUBNA}
\author{S.J.D. Kay}\affiliation{\YORK}
\author{M. Korolija}\affiliation{\ZAGREB}
\author{B. Krusche}\affiliation{\BASEL}
\author{A. Lazarev}\affiliation{\DUBNA}
\author{K. Livingston}\affiliation{\GLASGOW}
\author{S. Lutterer}\affiliation{\BASEL}
\author{I.J.D. MacGregor}\affiliation{\GLASGOW}
\author{R.G. Macrae}\affiliation{\GLASGOW}
\author{D.M. Manley}\affiliation{\KENT}
\author{P.P. Martel}\affiliation{\MAINZ}\affiliation{\MOUNTALLISON}
\author{R. Miskimen}\affiliation{\MASSACHUSETTS}
\author{M. Mocanu}\affiliation{\YORK}
\author{E. Mornacchi}\affiliation{\MAINZ}
\author{C. Mullen}\affiliation{\GLASGOW}
\author{A. Neganov}\affiliation{\DUBNA}
\author{A. Neiser}\affiliation{\MAINZ}
\author{M. Oberle}\affiliation{\BASEL}
\author{M. Ostrick}\affiliation{\MAINZ}
\author{P.B. Otte}\affiliation{\MAINZ}
\author{D. Paudyal}\affiliation{\REGINA}
\author{P. Pedroni}\affiliation{\PAVIAINFN}
\author{A. Powell}\affiliation{\GLASGOW}
%\author{S.N. Prakhov}\affiliation{\LA}
\author{G. Reicherz}\affiliation{\BOCHUM}
%\author{G. Ron}\affiliation{\JERUSALEM}
\author{T. Rostomyan}\affiliation{\BASEL}
%\author{A. Sarty}\affiliation{\HALIFAXCANADA}
\author{C. Sfienti}\affiliation{\MAINZ}
\author{V. Sokhoyan}\affiliation{\MAINZ}
\author{O. Steffen}\affiliation{\MAINZ}
\author{I.I. Strakovsky}\affiliation{\WASHINGTON}
\author{T. Strub}\affiliation{\BASEL}
\author{I. Supek}\affiliation{\ZAGREB}
\author{A. Thiel}\affiliation{\HISKP}
\author{M. Thiel}\affiliation{\MAINZ}
\author{A. Thomas}\affiliation{\MAINZ}
\author{Yu.A. Usov}\affiliation{\DUBNA}
\author{S. Wagner}\affiliation{\MAINZ}
\author{N.K. Walford}\affiliation{\BASEL}
\author{D.P. Watts}\affiliation{\YORK}
\author{D. Werthm\"uller}\affiliation{\YORK}
\author{J. Wettig}\affiliation{\MAINZ}
\author{L. Witthauer}\affiliation{\BASEL}
\author{M. Wolfes}\affiliation{\MAINZ}
\author{N. Zachariou}\affiliation{\YORK}
%\author{L.A. Zana}\affiliation{\JLAB}


%\author{L.~Witthauer \dots}\affiliation{\BASEL}

\collaboration{A2 Collaboration at MAMI}
 \vskip 0.25cm

%


